Towards Scalable Foundation Model for Multi-modal and Hyperspectral Geospatial Data

Geospatial raster data, such as that collected by satellite-based imaging systems at different times and spectral bands, hold immense potential for enabling a wide range of high-impact applications. This potential stems from the rich information that is spatially and temporally contextualized across multiple channels and sensing modalities. Recent work has adapted existing self-supervised learning approaches for such geospatial data. However, they fall short of scalable model architectures, leading to inflexibility and computational inefficiencies when faced with an increasing number of channels and modalities. To address these limitations, we introduce Low-rank Efficient Spatial-Spectral Vision Transformer with three key innovations: i) the LESS Attention Block that approximates high-dimensional spatial-spectral attention through Kronecker's product of the low-dimensional spatial and spectral attention components; ii) the Continuous Positional-Channel Embedding Layer that preserves both the continuity and physical characteristics of each spatial-spectral patch; and iii) the Perception Field Mask that exploits local spatial dependencies by constraining attention to neighboring patches. To evaluate the proposed innovations, we construct GFM-Bench, which serves as a comprehensive benchmark for such geospatial raster data. We pretrain LESS ViT using a Hyperspectral Masked Autoencoder framework with integrated positional and channel masking strategies. Experimental results demonstrate that our proposed method achieves competitive performance against state-of-the-art multi-modal geospatial foundation models while outperforming them on cross-satellite generalization tasks with higher computational efficiency. The flexibility and extensibility of our framework make it a promising direction for future geospatial data analysis tasks that involve a wide range of modalities and channels.

==> tables/efficiency.tex <==
\begin{table}[t]
\centering
    \caption{\textbf{Model Efficiency.} We analyze computational efficiency across architectures by comparing model parameter counts, floating point operations (FLOPs) during fine-tuning, and time requirements for both fine-tuning and inference on BigEarthNet~\cite{ben}. To enable direct comparison, we normalize both FLOPs and wall-clock times relative to LESS ViT's baseline measurements. The mAP of each experiment is also reported.}
    \label{tab:efficiency}
    \footnotesize
    \renewcommand{\arraystretch}{1.2} % Adjust row height
    % \setlength{\tabcolsep}{1pt} % Adjust column separation
    \resizebox{0.7\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Architecture} & \textbf{\# Param.} & \textbf{Fine-Tuning Time} & \textbf{\# FLOPs} & \textbf{Inference Time} & \textbf{mAP}\\ \midrule
ViT~\cite{satmae}          & 86.1M     & $\times0.2$   & $\times0.6$  & $\times 0.1$    &\textbf{87.57}\\
Channel-ViT~\cite{channel_vit} & 85.4M     & $\times3.3$  & $\times2.4$ &$\times2.0$ & 80 \\
\bluerow LESS ViT     & 83.2M     & $\times1.0$ & $\times1.0$   &$\times1.0$ & 86.08\\
\bottomrule
\end{tabular}
}
\end{table}
